End-to-end Optimization of Machine Learning Prediction Queries

Prediction queries are widely used across industries to perform advanced analytics and draw insights from data. They include a data processing part (e.g., for joining, filtering, cleaning, featurizing the datasets) and a machine learning (ML) part invoking one or more trained models to perform predictions. These parts have so far been optimized in isolation, leaving significant opportunities for optimization unexplored. We present Raven, a production-ready system for optimizing prediction queries. Raven follows the enterprise architectural trend of collocating data and ML runtimes. It relies on a unified intermediate representation that captures both data and ML operators in a single graph structure to unlock two families of optimizations. First, it employs logical optimizations that pass information between the data part (and the properties of the underlying data) and the ML part to optimize each other. Second, it introduces logical-to-physical transformations that allow operators to be executed on different runtimes (relational, ML, and DNN) and hardware (CPU, GPU). Novel data-driven optimizations determine the runtime to be used for each part of the query to achieve optimal performance. Our evaluation shows that Raven improves performance of prediction queries on Apache Spark and SQL Server by up to 13.1x and 330x, respectively. For complex models where GPU acceleration is beneficial, Raven provides up to 8x speedup compared to state-of-the-art systems.

==> background.tex <==
\section{Preliminaries}
\label{sec:background}

In this section, we provide background on prediction pipelines, and discuss their execution and optimization, the later being the focus of this paper.

Prediction pipelines are advanced analytics queries that use ML models to perform predictions. They receive as input data residing in files (e.g., local files, cloud stores, or data lakes) or databases.
We find that big part of the data for predictions in the enterprise are either structured or semi-structured, hence they are often stored in (relational) databases. \kk{citation here}

\KK{Motivate the existence of pipelines from Fotis' GH datasets.}

\kk{Introduce onnx. ONNX is worth mentioning as a recent attempt for an open format to standardize ML model representation in an engine-agnostic manner, similar to the role of relational algebra in RDBMSs}

Within a prediction pipeline, data is first processed, e.g., to combine different tables/datasets, clean them, or perform featurization through scaling and encoding. Once processed, this data is fed to one or more models. ML models are typically authored in one of the popular ML frameworks, such as scikit-learn, PyTorch, TensorFlow, SparkML, ONNX. The data operations were typically done either in SQL or in Python (e.g., using Pandas). SQL is common for data that reside in the database (but not necessary). As data processing is a central part of invoking models, most ML frameworks added support for data operations: \kk{examples here.} What ends up happening is that people have started using them but still use SQL or Python. So part of the pre-processing can be in the model pipeline and part before it in SQL/Python.
\mi{I think that what is missing here is the training vs inference explanation. As it reads now there is no mention to training and this may confuse readers.}
\mi{Maybe we can also frame the problem differently. What data scientist to now is a bunch of data-preprocessing using SQL e.g., filter, joining, etc. Then they export the data from the dataset into flat file (e.g., CSV) and then they open their python environemt and build pipelines composed of data featurizers and models. They train the pipelines. Afterwards, they need to deploy the trained pipelined as well as the sql query on new fresh data for prediction. Raven optimizes the case in which the input data is either inside a database e.g., SQL Server, or distributed over machines e.g., using Spark. Blabla}
\kp{We are targeting data in DBMS now, but the core technique can be applied to Python pandas as well I think. e.g., optimize ML model and use it with reduced # of inputs.}
We observe two main ways to express pipelines: either through SQL or through Python. In this work, we focus on the SQL syntax as adopted by SQL Server offerings (including Azure SQL DB and DW~cite{dwml}). Similar SQL-based syntaxes have been used by both Google BigQueryML and Amazon RedshiftML. However, as we will show in \autoref{sec:ir}, we have ongoing work to support pipelines expressed in Python---it is all about translating them to our unified IR. Then the rest will work as is.

We consider ONNX models, and by transitivity models that can be convertered to ONNX. Other models can easily be expressed in our IR.
Note also that we focus on traditional ML models, such as linear regressions, decision trees, and forests, as our optimizations target those at the moment (but we support the execution of any model). \kk{Support importance of traditional ML. Also citations from HB.}


\kk{Describe in more detail running example here.}


\KK{How many people are using SQL+PREDICT.}

\KK{Can we claim sth about using Scope data with data transformations? Ryder McMinn is doing a lot of that. He talked about joins and group bys happening a lot.}

% Data for performing inference are rarely ready to be directly fed to ML models in practice.
% Joining/unioning of multiple datasets, data cleaning (e.g., imputation), and featurization (e.g., scaling, encoding of categorical features) are very often performed to prepare the data that are then used for inference using the models.


% Data scientists and developers use various ways today for expressing inference pipelines.
% One common way is to use Python (other through Pandas) for the data processing part that is then used to invoke the model expressed in an ML framework (e.g., scikit-learn, TensorFlow, PyTorch). The importance of expressing inference pipelines is exhibited by the fact that various frameworks are adding native support for them: scikit-learn pipelines, various data operations in ONNX and TensorFlow \KK{links here}.
% Another approach is to use SQL for the data processing and then an integrated feature for performing inference (e.g., PREDICT in SQL Server or a UDF in Redshift, MADlib).
% Essentially in-DB model inference was motivated, among others, by such pipelines that perform heavy data operations.



% Data scientists and developers use various ways today for expressing inference pipelines.
% One common way is to use Python (othen through Pandas) for the data processing part that is then used to invoke the model expressed in an ML framework (e.g., scikit-learn, TensorFlow, PyTorch). The importance of expressing inference pipelines is exhibited by the fact that various frameworks are adding native support for them: scikit-learn pipelines, various data operations in ONNX and TensorFlow \kk{links here}.
% Another approach is to use SQL for the data processing and then an integrated feature for performing inferecence (e.g., PREDICT in SQL Server or a UDF in Redshift, MADlib).
% Essentially in-DB model inference was motivated, among others, by such pipelines that perform heavy data operations.

\KK{Give better links and data (e.g., thru Fotis' notebooks) for inference pipelines.}


\mypar{Execution of prediction pipelines}

Mention in-DB style (e.g., PREDICT in SQL Server or a UDF in Redshift, MADlib).
Then there is the Python-based. Say about what we are doing with in-DB and Spark.

In this paper we focus on the optimization of 
Make clear the focus of this paper.

\mypar{Optimization of inference pipelines and \sysname}
In terms of optimizations, we have all the DB optimizers and separately ML optimizers, but nothing that combines both.
Weld is an exception---any other and why not enough?
Talk about Weld (physical optimizations as opposed to Raven's logical---complimentary). Willump does cascading of models---also complimentary.


